A-NeRF: Articulated Neural Radiance Fields for Learning Human Shape, Appearance, and Pose

While deep learning reshaped the classical motion capture pipeline with feed-forward networks, generative models are required to recover fine alignment via iterative refinement. Unfortunately, the existing models are usually hand-crafted or learned in controlled conditions, only applicable to limited domains. We propose a method to learn a generative neural body model from unlabelled monocular videos by extending Neural Radiance Fields (NeRFs). We equip them with a skeleton to apply to time-varying and articulated motion. A key insight is that implicit models require the inverse of the forward kinematics used in explicit surface models. Our reparameterization defines spatial latent variables relative to the pose of body parts and thereby overcomes ill-posed inverse operations with an overparameterization. This enables learning volumetric body shape and appearance from scratch while jointly refining the articulated pose; all without ground truth labels for appearance, pose, or 3D shape on the input videos. When used for novel-view-synthesis and motion capture, our neural model improves accuracy on diverse datasets. Project website: https://lemonatsu.github.io/anerf/ .

==> acknowledgement.tex <==
\subsection{Acknowledgements}

Shih-Yang Su, Frank Yu and Helge Rhodin were supported by Compute Canada and Advanced Research Computing at the University of British Columbia~\cite{sockeyearc}.



==> checklist.tex <==
\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{At the end of Section 4.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{At the end of Section 1.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We will release the code upon acceptance with detailed explanation.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Details are provided in the main document and further ones given in the supplementary materials.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{We experimented on Human 3.6M S9 Protocol~\RNum{2} with 3 different random seeds. We trained for 100k iterations each, and the resulting PA-MPJPE difference is negligible ($\leq0.03$). We did not report this in the paper.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{All datasets in the papers are free for academic use.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> figures/method/input_rep.tex <==
\newlength\inputrepscale
\setlength\inputrepscale{0.245\linewidth}
\begin{figure}[t]
\centering
\setlength{\fboxrule}{0pt}%
\parbox[t]{\inputrepscale}{%
\vspace{0mm}\centering%
\fbox{\includegraphics[width=\inputrepscale,trim=50 80 20 40,clip=true]{images/method/input_rep/querypts_none}}\\%
{\footnotesize(a) Query~Point + Joint~Positions}
}%
\parbox[t]{\inputrepscale}{%
\vspace{0mm}\centering%
\fbox{\includegraphics[width=\inputrepscale,trim=50 80 20 40,clip=true]{images/method/input_rep/querypts_relview}}\\%
{\footnotesize(b) Query~Point + Joint~Positions  + Rel.~Dir. + Rel.~Ray}
}%
\parbox[t]{\inputrepscale}{%
\vspace{0mm}\centering%
\fbox{\includegraphics[width=\inputrepscale,trim=50 80 20 40,clip=true]{images/method/input_rep/reldist_relview}}\\%
{\footnotesize(c) Rel.~Dist. + Rel.~Dir. + Rel.~Ray  }
}%
\caption{\tb{Encoding ablation study on a novel view.}  (a) Directly applying positional encoding on the concatenation of query point $\query$ as in NeRF is unsuitable for learning pose-dependent models, even when conditioning on the skeleton joint locations. Also when encoding only the directional information (b) or distances and view-ray direction relatively (c) artifacts remain. 
(d) Our Pose-relative representation drastically improves the quality of the articulated human representation.
}
\label{fig:input-rep}
\end{figure}


==> figures/method/multi_view.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.66\linewidth]{images/method/multi-view-out.png}
\caption{\tb{Multi-view setup.} Our A-NeRF learning and test-time pose refinement method naturally generalizes to multiple views. For every frame, a single view-consistent neural radiance field (center) as well as underlying 3D skeleton pose is reconstructed. The camera pose is estimated and refined for every frame and view automatically. Faces in H3.6M images blurred for anonymity.}
\label{fig:multi-view}
\end{figure}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> method_old.tex <==
\section{Method}
\input{overview}
\subsection{Skeleton Pose Initialization}
\label{sec:data-prepreoc}
Our skeleton representation follows that of SMPL~\cite{loper2015smpl}, but without the associated parametric surface model. Our representation consists of two elements: (i) a skeleton structure in a rest pose of $m=24$ 3D joint locations $\{\jointele_i\}_{i=1}^m$, with the root at $\mathbf{0}$, and (ii) the per-image skeleton poses $\smplpose_k=\veclistkiz{\smplbone}{24}$ that include the relative rotation of 24 joints, $\subki{\smplbone}$, in the recently proposed overparametrized representation of \cite{zhou2019continuity} ($\subki{\smplbone} \in\smplbonespaceNEW$). 
We use the subscript $(k,i)$ to indicate that a variable is related to the $i$-th joint of image $\mI_k$. The rotation $\subki{\smplbone}$ determines the relative orientation of a bone to its parents. 
We refer to the coordinate system spanned by the joint rotation axis $\subki{\smplbone}$ and vector between $i$ and its parent as local bone coordinates. The 3D world coordinates $\vq \in\jointelespace$ of a point $\subki{\vp} \in\jointelespace$ in the $i$-th local bone coordinates is then computed with forward kinematics using homogeneous coordinates,
\begin{align}
\hmvec{\vq} &= \jointtrans\, \hmvec{\vp}, 
\end{align}
 with the $4\times4$ local-to-world transformation matrix
\begin{align}
\jointtrans &= \prod_{j\in A(i)}\begin{bmatrix}
\mR(\subkj{\omega}) & \jointele_j \\ 
\mathbf{0} & 1
\end{bmatrix},\label{eq:joint-transform}
\end{align}
$\mathbf{0}=\left[0,0,0\right]$, $A(i)$ is the ordered set of the joint ancestors of $i$, and $\mathbf{\jointele}_i\in\jointelespace$ the joint location of $i$ at the rest pose. The rotation matrix $\mR(\subkj{\omega})$ is inferred as in~\cite{zhou2019continuity}.
We acquire the initial skeleton poses $\theta_k$ and the estimated camera matrix $\cameramatrix_k$ for image $\mI_k$ using SPIN~\cite{kolotouros2019learning_spin}, a state-of-the-art single image 3D human pose and shape estimator. Since SPIN predicts $\mathbf{\jointele}_i\in\jointelespace$ for every image, we average the rest pose over all $k$ to obtain consistent bone length estimates. 


\subsection{A-NeRF---Setting and Pose Refinement Objective}
\label{sec:joint refinement}

Our goal is to learn a volumetric body model parametrized by $\phi$ and to optimize the agreement of its rendering $\render(\smplpose_k)$ on the set of images $\{\mI_k\}^n_{k=1}$ with respect to the underlying skeleton pose $\smplpose_k$. Formally, we write the joint modeling and reconstruction objective
\begin{equation}
\cL^\text{SV}(\smplpose, \phi) = \sum_k d(\render(\smplpose_k), \mI_k) + \lambda d(\smplpose_k,\hat{\smplpose}_k),
\label{eq:objective}    
\end{equation}
where $\nerfparam$ are the parameters of a neural network defining density and radiance of a volume, $\render$ is a classical volumetric renderer that ray casts the neural volume, $\hat{\smplpose}_k$ is the initial pose estimate from SPIN, $\lambda$ is a hyperparameter that controls the regularization strength, and $d$ is a distance function, %
such as the $l_1$ distance. 

This objective is optimized using stochastic gradient descent. In other words, we jointly train the neural network parameters $\nerfparam$ that define how the body model is rendered given pose $\smplpose_k$ as well as refine the pose $\smplpose_k$ such that the same model $\nerfparam$ can explain each image $\mI_k$. The last term $\lambda d(\smplpose_k,\hat{\smplpose}_k)$ controls the amount of changes to apply to the initial estimate $\hat{\smplpose}_k$.
How pose and model are linked is explained in the following sections.

\paragraph{Assumptions} We assume that the images $\mI_k$ stem from one or multiple videos of the same person captured with static cameras. 
In the most general case, the input is a monocular video but we also provide an extension that imposes multi-view constraints if multi-view footage is available. We distinguish the single-view and multi-view case with $\cL^\text{SV}$ and $\cL^\text{MV}$, respectively. Notably, we do not require intrinsic or extrinsic camera calibrations in either of these settings. This is different from many structure-from-motion approaches, which explicitly require camera motion with a strong translation component to calibrate; impractical for casual recordings.
This uncalibrated setup drastically eases setup time compared to existing solutions that operate in the same accuracy range.

Most importantly, the neural body model $\nerfparam$ is learned from scratch, no parametric actor model nor separate model calibration step is required, which additionally eases its application. The steps required to attain this level of automation are explained in the following.

\subsection{Volumetric Rendering with Neural Radiance Fields}
\label{sec:NeRF}

Our rendering model follows that of NeRF~\cite{mildenhall2020nerf}, with only minor additions to the importance sampling that improve the effectiveness by exploiting the estimated initial skeletal pose $\theta$.

NeRF stores the density $\density$ and radiance $\rgb$ of a 3D point $\query$ in view direction $\viewdir$ using a 10-layer fully-connected neural network  $(\density,\rgb)=\nerffunc(\query,\viewdir)$ with $946500$-dimensional parameters $\nerfparam$. Similar to classical frequency-space embeddings of volumetric data, this yields a compact parametric representation of the scene that can be ray-cast by sampling $\query$ along the view direction $\viewdir$. NeRF attained a breakthrough by using positional encoding, the projection of the query 3D position onto a high number of spatial sine and cosine waves of varying wavelengths. Conditioning on this high-dimensional space encourages the learning of low and high frequency features. 


This neural density and radiance field is then formed into an image by ray casting. Each ray emitted from the camera is first sampled at 64 points and $\nerffunc$ is evaluated at each.
The samples together form a piece-wise constant probability density function (PDF) that is integrated using the Beer-Lambert law. A pixel at coordinate $(u,v)$ is rendered as

\begin{align}
\render(u,v) &= \sum_i T(x_i)(1-\exp(-\density(x_i)\delta(x_i)))\rgb(x_i), \text{ with }\\
T(x_i)&=\exp(-\sum_{j=1}^{i-1}\density(x_i)\delta(x_j)),
\label{eq:image fromation}
\end{align}
and $x_i$ the sample points, $\delta(x_i)$ the distance between $x_i$ and $x_{i+1}$, and $T(x_i)$ the accumulated transmittance for the ray traveling from the near plane to $x_i$.%

At training time, the neural network parameters $\nerfparam$ are optimized by minimizing the distance between the rendered pixel color $\render(u,v)$ and the true image color $\mI(u,v)$ at pixel coordinate $(u,v)$. In essence, the image formation function, which is differentiable, takes the role of a fixed-pipeline neural network layer that connects to the underlying NeRF network. It facilitates end-to-end training of the network parameters $\nerfparam$, which subsequently encode the radiance and density of the entire scene and can be rendered from novel views by changing the virtual camera (view direction $\viewdir$).

We follow the original work in using a coarse-to-fine training strategy. A second neural network $\nerffunc'$ is learned by sampling 16 additional samples from the piecewise-constant PDF inferred from the 64 initial samples and repeating the above rendering with the 64+16 locations. Since both neural networks have the same structure and function and are trained and evaluated in sequence, we make no distinction in the following.

However, the original NeRF formulation was designed to reconstruct a single static scene from a massive number of calibrated views, which is not applicable to our setting of a moving person unless captured in a camera dome. Straight-forward extensions that we tried, such as conditioning $\nerffunc$ on the frame or initial pose estimate $\theta$ fail in that the neural network either memorizes all the possible mappings of $(\density,\rgb)\leftarrow(\theta,\query,\viewdir)$ from a small training set and degrades into fog-like artifacts when the number of training poses increases. It generalizes poorly not just to unseen human poses, but also to shifted or rotated training poses, as shown in ~\figref{fig:example-shift} and~\secref{sec:ablation}.

\subsection{A-NeRF---Pose-Relative Embedding}
\label{sec:input-pre}
\input{figures/method/input_rep}

Motivated by the observation that the positional encoding in terms of frequency components in NeRF was a game changer, we derived a novel embedding that is tailored for articulated human motion. 
The idea is to define the model density and radiance relative to the rigid bones of the skeleton instead of explicitly conditioning on skeleton pose. Although not providing additional information to the neural radiance field, this creates an implicit bias that encourages the network to store only that information in relation to bone $j$ that is influenced by $j$. Embedding information of other joints would not be consistent under relative pose changes; thereby, discouraging dependencies due to the increased complexity of relations.

In the following, we introduce five skeleton-relative embedding variants that replace the positional encoding in Euclidean space explained in the previous section. Each of them first maps the 3D query point $\vx$ via the inverse of the bone-to-world transformation $\jointtrans$ explained in Section~\ref{sec:data-prepreoc}. Formally we write
\begin{equation}
\hmvec{\subki{\local{\query}}} = \jointtransinv\hmvec{\query}.
\label{eq:world to bone}
\end{equation}
An overview of all embeddings is given in ~\figref{fig:input-rep}.


\subsubsection*{Relative Positional (Rel. Pos.) encoding.}
The query point $\vx$ is mapped to all bones of the skeleton with Equation~\ref{eq:world to bone}. Because we perform positional encoding afterwards as in the original NeRF, this blows up the already massive positional encoding space by a factor of the number of joints (for us 24), drastically increasing the memory footprint. 

To this end, we propose the following alternatives. Two for encoding the query position and two for the view direction.

\subsubsection*{Relative Distance (Rel. Dist.) encoding.} Given $\smplpose_k$, we calculate the $l_2$ distance from the 3D query point $\query$ to joint $i$ by
\begin{align}
    \subki{\querydist} &= \norm{\subki{\local{\query}}}_2.%
\end{align}
Recall, $\subki{\local{\query}}$ is $\query$ in the local coordinate of joint $i$. Storing only the distance reduces input parameters by a factor of three.

\subsubsection*{Relative Direction (Rel. Dir) encoding.}
Since the distance maps many 3D points to the same scalar, we additionally obtain the direction vector to capture the orientation information of $\query$ by
\begin{equation}
\queryrot^\mI_k=\frac{\subki{\local{\query}}}{\norm{\subki{\local{\query}}}_2}.    
\end{equation}
We do not apply positional encoding on this direction encoding, which dramatically saves network capacity.

\subsubsection*{Relative Ray Direction (Rel. Ray.) encoding.}
NeRF builds upon a radiance field that is a function of the position and view direction. To encode the view direction, we transform $\viewdir$ to obtain the relative view-ray direction $\local{\viewdir}$ by applying the rotational part of the bone-to-world transformation $\jointtrans$,
\begin{equation}
\local{\viewdir} = [\jointtransinv]_{3\times 3} \viewdir,
\label{eq:world to bone rot}
\end{equation}
with $[\jointtransinv]_{3\times 3}$ the top-left $3\times 3$ submatrix.

\subsubsection*{Relative Ray Angle (Ray. Angl.) encoding.} The other view-direction encoding we explore is the angle between the ray $\viewdir$ and the vector $\vu$ from query point to joint origin,
\begin{equation}
\viewdir' = \text{arc cos}(\viewdir \bullet \vu),
\end{equation}
with $\bullet$ the dot product. As the distance encoding for position, this encoding has the advantage of being one-dimensional.

These relative embeddings have the advantage of being invariant to global shift and rotation of the person and preserve the piece-wise rigidity of articulated motion while still allowing for pose-dependent deformation. The handling of view-dependent illumination effects is explained in the extensions section (Section~\ref{sec:extensions}).

\subsection{A-NeRF---Pose-Relative Rendering and Learning}
\label{sec:A-NeRF}

With our relative skeleton embeddings introduced, we now turn to defining our Articulated NeRF Rendering model that is tailored to modeling human shape and appearance and lends itself for pose refinement of the underlying skeleton.

In a first step, we leave the NeRF model as is and only change the input to the neural network that encodes the radiance field used for volumetric rendering. We will expand on further extensions in the subsequent section. Samples along each view ray are taken as before (see Section~\ref{sec:NeRF}), however, now each query point is mapped to each of the $n=24$ bone coordinate systems and projected to the previously introduced encodings. This yields vectors $\querydist=\veclistki{\querydist}{24}$, $\queryrot=\veclistki{\queryrot}{24}$ and $\local{\viewdir}=\veclistki{\local{\viewdir}}{24}$, that are fed into the neural radiance field function
\begin{align}
(\density,\rgb)=\nerffunc(\querydist,\queryrot,\local{\viewdir}).
\label{eq:relative-nerf}
\end{align}
Image formation (Eq.~\ref{eq:image fromation}) takes in the output of this re-parametrized NeRF but remains unchanged otherwise.

The effect is that density and radiance values are now stored relative to the skeleton parametrized by $\smplpose$. Changing the skeleton parameters changes the local bone coordinate systems and therefore the density and radiance with them---like a manually rigged character would behave. This conditioning on pose allows us to optimize $\cL^\text{SV}$, our objective (Eq.~\ref{eq:objective}), jointly with respect to pose $\smplpose$ and neural network weights $\nerfparam$ that define the radiance field.

It is a-priori unclear whether this joint optimization can succeed, in fact, our initial experiments on conditioning NeRF on pose explicitly did not. The employed neural network is a general function approximator that has the degrees of freedom to compensate to give the same output for two different configurations of $\smplpose$. Nevertheless, our experiments show that our complete method can jointly refined pose from an off-the-shelf pose estimate. The learned model is not only consistent and visually accurate but better matches the ground truth 3D pose. 

We believe that our skeleton-relative encodings make learning feasible because they induce an implicit bias to the learning of the MLP, much like the invariance of convolutions, which helps CNNs to learn from images.


\paragraph{Relation to existing pose embeddings.}

An alternative would be to define the NeRF field in a reference pose and to map query points to this template. While this works well for points on or close to a surface \cite{taylor2012vitruvian,huang2020arch} and small deformation fields~\cite{park2020arxiv_deformablenerf}, it is ill-posed for articulated motion. For instance, when left and right hand are close a nearby query point can not be uniquely attributed to the left or right side. 


\subsection{Extensions}
\label{sec:extensions}

We propose several extensions that make Articulated NeRF computationally tractable and more accurate.

\subsubsection*{Sparse sampling and gradient accumulation} At training time, we form a batch of rays by randomly sampling 2048 rays from all available images. Therefore, not every frame will be optimized in every iteration. Moreover, every frame that is included may only be sampled with a few rays. As a result, optimizing the $\smplpose$ at every iteration is prone to noise in the stochastic gradient estimate. To counteract, we accumulate the gradient update $\Delta \smplpose$ for 50 iterations before updating. Without this, pose refinement diverged in our experiments.

\subsubsection*{Background handling.} In addition, to make our network focus on learning the subject's representation, we provide the renderer with the background image $B$ obtained as the median pixel value over all images taken from the same camera, exploiting the constant background assumption. Let $a(x_i)=T(x_i)(1-\exp(-\density(x_i)\delta(x_i)))$, the render outputs at $(u,v)$ becomes
\begin{equation}
\render(u,v) = \left(1-\sum_ia(x_i)\right)B(u,v)+\sum_i a(x_i)\rgb(x_i),
\label{eq:renderer}    
\end{equation}
with the background filling that fraction of light that passes through the entire volume.

\subsubsection*{Sampling optimization.} 
To further increase the sampling efficiency, we define a cylinder surrounding the initial skeleton pose estimate and sample points along the ray segment that lies inside. This is sketched in Figure~\ref{fig:overview}. Moreover, we use the background estimate to segment the person and only sample rays inside. Because this estimate is uncertain, we dilate the initial segmentation by 3 pixels.


\subsubsection*{Positional Encoding with Cutoff}
\label{sec:posenc}
\input{figures/method/cutoff_illustration}
To capture the high frequency details from the training images $\left\{\mI_k\right\}_{k=1}^{n}$, prior works incorporate periodic activation functions~\cite{sitzmann2020implicit_siren} in their neural networks, or adding high frequency input components~\cite{tancik2020fourfeat,mildenhall2020nerf}. We follow the latter approach in our work. Specifically, we adopt a weighted version of positional encoding~\cite{mildenhall2020nerf,vaswani2017attention_transformer}
\begin{equation}
\begin{split}
    \gamma(p,w) = w\bigg[p,&\pesin{0}{p},\pecos{0}{p},\cdots, \\
                 &\pesin{L-1}{p},\pecos{L-1}{p}\bigg],
\end{split}
\end{equation}
where $L$ is the number of frequency components, and $w$ is the weighting factor. We calculate $w$ as a per-joint weighting factor that depends on the distance $\subki{\querydist}$
\begin{equation}
\subki{w}=\begin{cases}
1., & \text{if } \subki{\querydist} \leq t\\
\exp\left(-\frac{1}{2s^2}\left(\subki{\querydist}-t\right)^2\right), & \text{otherwise}.
\end{cases}
\end{equation}
Here, $t$ denotes a cutoff threshold, and $s$ is a hyperparameter controlling how fast the Gaussian weight should be reduced to 0 as $\subki{\querydist}$ increases. We apply $\gamma$ on the relative distance $\subki{\querydist}$ and view direction $\subki{\local{\viewdir}}$ of all joints $i$ such that
\begin{align}
    \querydist=\left[\wpe{\querydist}{1},\cdots,\wpe{\querydist}{24}\right],\\
    \local{\viewdir}=\left[\wpe{\local{\viewdir}}{1},\cdots,\wpe{\local{\viewdir}}{24}\right].
\end{align}
The intuition behind this weighted positional encoding is that if the joint $i$ is far away from $\query$ (i.e., has large $\subki{\querydist}$), its input encoding should have less influence on the output. Our empirical results show that the proposed encoding helps reduce noise in the background (\secref{sec:ablation}).


\subsubsection*{Appearance codes} Illumination effects such as shadows and shading depend on the view direction in relation to the light position in world coordinates. We encode the former relative to the skeleton, which however is invariant to global position. Following concurrent work on handling illumination changes \cite{martin2020arxiv_nerfiw}, we add a 16-dimensional appearance code to the second last layer of the NeRF network $\nerffunc$. It is individually stored and optimized for every frame. Due to its position at the end of the network and its low dimensionality, it helps learning these global effects while not deteriorating the benefits of the relative encoding.

\subsubsection*{Multi-view constraints}
\input{figures/method/multi_view}

We can further incorporate a multi-view constraint to improve pose refinement when the motion is captured from multiple cameras. \figref{fig:multi-view} shows the two camera case that is most practical. For initializing $\smplpose_k$, we average the individual joint rotation estimates from all $V$ views $v \in [1, \dots, V]$. Since rotations are relative to the parent and root, this works without calibrating the cameras. Only the global position and orientation remains specific to view $v$. To this end, we extend our single-view notation with subscripts, position $\smplbone^{(v)}_{k,1}$ and orientation $\smplbone^{(v)}_{k,2}$ are estimated relative to camera $v$.

For refinement, we extend the single view objective Eq.~\ref{eq:objective} to make $\smplpose_k$ view-consistent. With slight abuse of notation we write,
\begin{equation}
\cL^\text{MV}(\smplpose, \phi) = \sum_c \sum_k d(\render(\smplpose_k, \smplbone^{(v)}_{k,0}, \smplbone^{(v)}_{k,1}, \mK^{(v)}), \mI^{(v)}_k) + \lambda d(\smplpose_k,\hat{\smplpose}_k),
\label{eq:objective multiview}    
\end{equation}
with $\smplpose_k$ shared across all views $v$, except for the global skeleton position, $\smplbone^{(v)}_{k,0}$, and global orientation, $\smplbone^{(v)}_{k,1}$, which are estimated independently per camera view $v$ since the relative camera position and orientation is unknown in our setting. 


\subsubsection{Implementation details}
We train our A-NeRF for a total of 500k iterations: During the first 100k, we jointly update A-NeRF weights $\phi$ and refine pose estimates $\theta$ using the $l_1$ distance. We then stop optimizing $\theta$, and continue to train the A-NeRF model for improved visual fidelity additional 400k iterations using the $l_2$ distance. We use Adam optimizer~\cite{kingma2014adam}, and keep separate step sizes for A-NeRF and pose refinement. For A-NeRF, we start with step size $0.0005$ and exponentially decay it to $0.00005$. For pose refinement, we use a fixed step size of 0.001 throughout the joint optimization process, and set the regularization parameter $\lambda=2$, and the cutoff threshold $t=500$mm. The training is done on 1 Nvidia Tesla V100 32GB GPU, which takes approximately 60-70 hours. It takes around 8 seconds to render one $512\times512\times3$ image.

